MultiCol-SLAM - A Modular Real-Time Multi-Camera SLAM System

The basis for most vision based applications like robotics, self-driving cars and potentially augmented and virtual reality is a robust, continuous estimation of the position and orientation of a camera system w.r.t the observed environment (scene). In recent years many vision based systems that perform simultaneous localization and mapping (SLAM) have been presented and released as open source. In this paper, we extend and improve upon a state-of-the-art SLAM to make it applicable to arbitrary, rigidly coupled multi-camera systems (MCS) using the MultiCol model. In addition, we include a performance evaluation on accurate ground truth and compare the robustness of the proposed method to a single camera version of the SLAM system. An open source implementation of the proposed multi-fisheye camera SLAM system can be found on-line https://github.com/urbste/MultiCol-SLAM.

==> multislam_experiments_SLAM_features.tex <==
To evaluate the impact of the binary features developed in \SeeCh{ch:features}, we perform several experiments.
As depicted in \SeeTable{tab:ATESLAM} and \SeeTable{tab:RPEDELTA1} the features do not have a significant impact on the accuracy of the system.
First of all, the features use the same detector principle (FAST or AGAST respectively).
Thus the distribution of point in the images and the point localization accuracy is similar.
In addition, the standard ORB descriptor already leaves us with many points to track and the geometric verification and guided matching strategies ensure a sufficient number of points.

Still, the developed descriptors have some advantages over ORB.
Both, dBRIEF and mdBRIEF take only 16byte of storage compared to ORB which needs 32byte per descriptor.
At the same time, the tracking accuracy (\SeeTable{tab:ATESLAM}, \SeeTable{tab:RPEDELTA1}) and mean percent successfully tracked frames is equally good or better (\SeeTable{tab:SLamStatistics}).
At the same time, the additional computational cost is low enough to let the system operate in real-time.
The median timings (\SeeTable{tab:timingsSLAM}) for the mapping thread are slightly higher, as more points are matched and thus triangulated and adjusted.

In addition, we analyzed the distribution of tracked points per frame.
This is depicted in \SeeFig{fig:slam_nr_pts} for the two trajectories \textit{Laser 1} and \textit{Laser 2}.
The number of tracked points for dBRIEF and mdBRIEF is higher for most frames.
For trajectory \textit{Laser 2} it is obvious that mdBRIEF performs best.
MultiCol-SLAM with ORB features stopped tracking around frame 350 and is not able to recover, as the MCS moves only in one direction.
%evaluation:
%Outlier ratios
%relocalization speed recovery after loss
%features per frame
%dimension

\begin{figure*}
	\centering
	\subcaptionbox{Laser trajectory 1\label{fig:slam_nr_pts_per_frame_traj1}}
	{
		\begin{tikzpicture}[baseline=(current axis.south)]
		\begin{axis}[
		grid=major,
		ymax=150,ymin=0,
		xmin=0,xmax=1019,
		ylabel={\# tracked points / frame},
		xlabel={frame number},
		yticklabel pos=left,
		width = 0.4\textwidth,
		xtick={0,200,400,600,800,1000,1200},
		ylabel near ticks,
		xlabel near ticks,]
		\addplot+[no markers,color=red,line width=1pt]
		table [x index={0},y index={1}]  {images_and_data/multislam/results/pt_stats_multi.txt};
		\addplot+[no markers,color=blue,line width=1pt]
		table [x index={0},y index={2}]  {images_and_data/multislam/results/pt_stats_multi.txt};
		\addplot+[no markers,color=green,line width=1pt]
		table [x index={0},y index={3}]  {images_and_data/multislam/results/pt_stats_multi.txt};
		\end{axis}
		\end{tikzpicture}
	}\!
	\subcaptionbox{Laser trajectory 2\label{fig:slam_nr_pts_per_frame_traj2}}
	{
		\begin{tikzpicture}[baseline=(current axis.south)]
		\begin{axis}[
		grid=major,
		ymax=150,ymin=0,
		xmin=0,xmax=679,
		ylabel={\# tracked points / frame},
		xlabel={frame number},
		yticklabel pos=right,
		width = 0.4\textwidth,
		xtick={0,200,400,600},
		ylabel near ticks,
		xlabel near ticks,
		legend entries={ORB, dBRIEF, mdBRIEF},
		legend to name=legendSLAMPoints,
		legend columns=3]
		\addplot+[no markers,color=red,line width=1pt]
		table [x index={0},y index={1}]  {images_and_data/multislam/results/pt_stats_multi_traj2.txt};
		\addplot+[no markers,color=blue,line width=1pt]
		table [x index={0},y index={2}]  {images_and_data/multislam/results/pt_stats_multi_traj2.txt};
		\addplot+[no markers,color=green,line width=1pt]
		table [x index={0},y index={3}]  {images_and_data/multislam/results/pt_stats_multi_traj2.txt};
		\end{axis}
		\end{tikzpicture}
	}\\
	\begin{center}
		\ref{legendSLAMPoints}
	\end{center}
	\caption{Depicted is the number of tracked points for each frame for trajectories \textit{Laser 1} and \textit{Laser 2}.}
	\label{fig:slam_nr_pts}
\end{figure*}

==> multislam_experiments_model_supported.tex <==
\begin{table*}[]
	\centering
	%\resizebox{\textwidth}{!}{%
		\begin{tabular}{l|l|l|l|l|l|l|}
			\cline{2-7}
			& \multicolumn{3}{c|}{\textbf{ATE for MKFs}} & \multicolumn{3}{c|}{\textbf{RPE all frames}} \\ \cline{2-7} 
			& \multicolumn{3}{c|}{Multi-fisheye camera system} & \multicolumn{3}{c|}{Multi-fisheye camera system} \\ \cline{2-7} 
			& ORB & dBRIEF & mdBRIEF & ORB & dBRIEF & mdBRIEF  \\ \cline{2-7} 
			& {[}cm{]} & {[}cm{]} & {[}cm{]} & {[}cm{]}/{[}deg{]} & {[}cm{]}/{[}deg{]} & {[}cm{]}/{[}deg{]} \\ \hline
			\multicolumn{1}{|l|}{Laser 1} & 3.83 & 3.7  & 2.60 & 1.6/0.61 & 1.5/0.53 & 1.2/0.53  \\ \hline
			\multicolumn{1}{|l|}{Laser 2 fast} & 3.95 & 2.14 & 2.45 & 2.8/0.54 & 2.9/0.59 & 1.9/0.54 \\ \hline
		\end{tabular}
	%}%
	\caption{Median MKF \textbf{ATE}s and median RPEs for all frames for multi-camera \textbf{model-supported} tracking based on three different features descriptors.}
	\label{tab:ATEandRPEmodel}
\end{table*}

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{images_and_data/multislam/imgs/slam_and_modelbased_in_model.png}
\caption{Depicts three different trajectories transformed to the building model.
		The black trajectory is the ground-truth acquired by the lasertracker. The red trajectory represents the MultiCol-SLAM trajectory transformed to the ground truth trajectory by 7DOF alignment. The green trajectory is the trajectory estimated by the model-supported tracking method. During the fast 90$^\circ$ right turn, the SLAM trajectory starts to drift. This drift is avoided by tracking the model edges.}
\label{fig:model_support_vs_slam}
\end{figure*}
Finally, the model-supported tracking addition to MultiCol-SLAM presented in \SeeSec{ch:tracking:sec:modelintegration} is evaluated.
This is only possible for the trajectories \textit{Laser 1} and \textit{Laser 2}, as a building model is available.
To assess the performance and accuracies of our method, the initial MCS pose $\mathbf{M}_1$ is estimated from model points.
Subsequently, we perform the search for image edges described in \SeeSec{ch:tracking:sec:modelintegration} and optimize $\mathbf{M}_1$.
In addition, we re-calibrate the MCS by refining all transformation matrices $\mathbf{M}_c$ using the model edges.

The trajectory accuracies are depicted in \SeeTable{tab:ATEandRPEmodel}.
It is especially interesting to compare these values to the SLAM only evaluation of the trajectories presented in \SeeTable{tab:ATESLAM} and \SeeTable{tab:RPEDELTA1}.
From these results, it can be assumed that the building model has inferior accuracy compared to what the MCSs pose estimates are capable.
Indeed, the model-supported tracking RPE results are slightly inferior.
The ATE for the second trajectory however is over two times better.
The reason for this is, that the MCS makes a fast right turn at about half of the trajectory.
Here, the 'SLAM only' version starts to drift significantly and the scale of the reconstruction suffers.
As the trajectory contains no loops, the drift can not be corrected by propagating a loop closing error along the trajectory.
This is not the case for the model-supported trajectory estimate, as we always get robust MKF poses that are registered to model having an absolute frame.
This result is also qualitatively depicted in \SeeFig{fig:model_support_vs_slam}.



==> multislam_model_integration.tex <==
Thus far, the integration of the 3D model into our MultiCol-SLAM was only briefly mentioned in the mapping thread.
This section details the extraction of model edge and companion points and the search for corresponding image edges.

The model is supposed to support the tracking and mapping chain of our SLAM pipeline and help to classify points that are likely to be stable over time.
Such points could be used with a higher probability for re-localization.
In addition, the model provides scale information and images, e.g. taken for documentation, can be readily geo-referenced. 
In the following, we assume that the MCS localized itself in the building model using the methods presented in \cite{urban2013self}, thus the pose $\mathbf{M}_1$ of the first MKF w.r.t the model is known.

Different ways exist to integrate model information into the tracking process.
One can either perform model-based edge tracking either in an independent  pipeline or as a posterior refinement step of point-based frame to frame tracking.
As an alignment of each MCS pose to the model edges was not real-time capable, we decided to align only MKFs to the model and thus support the trajectory estimation.
Still, we use the pose of frame to frame point-based tracking as a prior.

In general, the goal is to align 3D model edges to edges extracted in the MCS images of a MKF.
First, we extract the model edge points $\mathbf{p}_e$ off-line, by analyzing the change of the normal vector between adjacent faces that a vertex is connected to. 
In this manner, we can identify vertexes that lie on a model edge.
The extracted edge vertexes are depicted in \SeeFig{subfig:modelPoints}.
In addition, we extract a companion point $\mathbf{p}_{co}$ for each edge vertex.
A companion point is the nearest vertex to $\mathbf{p}_e$ that also lies on the edge.
This second point is needed to estimate the orientation of the model edge projected into the images.

The image edges are extracted by first convolving each image of the MCS with a 3$\times$3 Sobel kernel.
Then the edges are thinned using Canny's method \cite{canny1986computational}.
An example is depicted in \SeeFig{subfig:cannyEdges}; 
For each edge pixel that remains after non-maximum suppression, we finally calculate the edge orientation $\phi_e$.

Then, for each new MKF, we project the model edge vertexes to the camera images. 
To retain only visible points, we use depth images that we render in advance.
To account for the pose uncertainty, we add a small offset (5cm) to the depth values.
Recall, that the initial pose estimate for the inserted MKF originates from point-based frame to frame tracking.
Thus generally, the projected model points $\mathbf{p}_e$ will not exactly lie on the images edges.
This is depicted in \SeeFig{subfig:projectedModelPts}.
Hence, we search along the edges normal direction for the corresponding image edge $\mathbf{m}'_{e}$.
This is depicted in \SeeFig{subfig:combinedEdgeAndSearch}.
The final measurements $\mathbf{m}'_{e}$ are depicted in green and the searched pixels are depicted by lines perpendicular to the projected model edges.
An edge is only accepted if the orientation difference is below some threshold.
The edge orientations are compared using the cosine similarity \SeeEq{eq:cosine}.

Finally, the pose is optimized by minimizing the reprojection error of the edge points $\mathbf{p}_e$.
The optimization is again carried out using MultiCol.

\begin{figure*}
	\centering
	\subcaptionbox{Model edge points $\mathbf{p}_e$\label{subfig:modelPoints}}{\includegraphics[width=0.49\textwidth]{images_and_data/multislam/imgs/modelPoints.png}}
	\subcaptionbox{Canny edges \label{subfig:cannyEdges}}{\includegraphics[width=0.49\textwidth]{images_and_data/multislam/imgs/cannyImg.png}}\par
	\subcaptionbox{Projected model points $\mathbf{p}_e$\label{subfig:projectedModelPts}}{\includegraphics[width=0.49\textwidth]{images_and_data/multislam/imgs/projectedModelPts.png}}	
	\subcaptionbox{Search lines and detected edge points $\mathbf{m}'_e$ \label{subfig:combinedEdgeAndSearch}}{\includegraphics[width=0.49\textwidth]{images_and_data/multislam/imgs/combined.png}}					
	\caption{Depicted is the process of detecting edge measurements for the model-supported tracking. (a) depicts the model edge vertexes $\mathbf{p}_e$. (b) depicts the Canny edge image of a real camera image. (c) depicts the projections of the map points $\mathbf{p}_e$ to the camera image using the MCS pose obtained by frame to frame point-based tracking. (d) depicts the search lines that are perpendicular to the edge directions. The edge directions $\phi_e$ are extracted using companion points $\mathbf{p}_{co}$ that are also projected to the image. The final edge measurements $\mathbf{m}'_e$ (green circles) are accepted if the angle between image edge and projected edge orientation is below some threshold.}
	\label{fig:modelEdgePtProjection}
\end{figure*}



%In this work, we basically use the mesh presented in  \SeeSec{ch:localization:sec:results} for all our experiments.
%Our methodology, however, is general and not limited to this particular model.
%A model consists of a set of vertexes, faces and normal directions for both entities.
%To render the model, the entire mesh is loaded and passed to the GPU.
%To align texture-less 3D models to images, edges are used.
%Thus, visible model edges have to extracted and sampled for each \gls{MKF}.
%One solution, would be to render normal and depth images and extract crease and step edges as done in \SeeCh{ch:localization:subsec:features}.
%As this yields thousands of edge pixels, the search for corresponding image edge pixels would take long.
%The number of edge pixels could be decreased by sub-sampling but still edge extraction has to be carried out for rendered and real images.
%Instead, we extract edge points model edge points $\mathbf{p}^e_i = [X_i,Y_i,Z_i]^T$ as well as a companion point $\hat{\mathbf{p}}_i = [X_i,Y_i,Z_i]^T$ for each edge point.
%A companion point is a point that is both the closed point to the edge point $\mathbf{p}^e_i = [X_i,Y_i,Z_i]^T$ and an edge point as well.
%$\mathbf{p}^e_i$ is used to estimate the edge orientation in the image.
